II. High Dimensional Estimation under Weak Moment Assumptions: Structured Recovery and Matrix Estimation

The purpose of this thesis is to develop new theories on high-dimensional structured signal recovery under a rather weak assumption on the measurements that only a finite number of moments exists. High-dimensional recovery has been one of the emerging topics in the last decade partly due to the celebrated work of Candes, Romberg and Tao (e.g. [CRT06, CRT04]). The original analysis there (and the works thereafter) necessitates a strong concentration argument (namely, the restricted isometry property), which only holds for a rather restricted class of measurements with light-tailed distributions. It had long been conjectured that high-dimensional recovery is possible even if restricted isometry type conditions do not hold, but the general theory was beyond the grasp until very recently, when the works [Men14a, KM15] propose a new small-ball method. In these two papers, the authors initiated a new analysis framework for general empirical risk minimization (ERM) problems with respect to the square loss, which is robust and can potentially allow heavy-tailed loss functions. The materials in this thesis are partly inspired by [Men14a], but are of a different mindset: rather than directly analyzing the existing ERMs for signal recovery for which it is difficult to avoid strong moment assumptions, we show that, in many circumstances, by carefully re-designing the ERMs to start with, one can still achieve the minimax optimal statistical rate of signal recovery with very high probability under much weaker assumptions than existing works.

==> chapter5/chapter5.tex <==
% Title page
%\addcontentsline{toc}{section}{\textbf{Title Page}}


% Dedication Page





\chapter{Statistical Rate of Recovery in Generative Models under Weak Moment Assumptions}
%\addcontentsline{toc}{chapter}{Abstract}
In this chapter, we consider estimating a high-dimensional vector from low dimensional measurements where the unknown vector is represented by a multi-layer Rectified Linear Units (ReLU) generative model $G:\mathbb{R}^k\rightarrow\mathbb{R}^d$ with $k\ll d$. Such a model poses structural priors on the unknown vector without having a dedicated basis, and in particular allows new and efficient approaches solving recovery problems with number of measurements far less than the ambient dimension of the vector. While progresses have been made recently regarding theoretical understandings on the linear Gaussian/sub-Gaussian measurements, much less is known when the measurements are heavy tailed.  
We show that, building upon the small-ball idea from Mendelson, one can in fact obtain a near optimal statistical rate in the presence of generative ReLU network under much weaker assumptions than sub-Gaussian measurements.

\section{Introduction and related works}
Consider a random pair $(\mathbf x, y)\in\mathbb R^d\times \mathbb R$ with the distribution satisfying the following model:
\begin{equation}\label{eq:model}
y = \dotp{\mf x}{G( \theta ^*)} + \xi,
\end{equation}
where $ \theta ^*\in\mathbb R^k$, the vector $\mf x\in\mathbb{R}^d$ is a random vector following a probability density $p(\mf x)$, $\xi$ is a random noise variable assumed to be independent of $\mf x$, and $y$ is the response variable.  The function $G:\mathbb{R}^k\rightarrow\mathbb{R}^d$ is a multi-layer ReLU network of the following form:
\begin{equation}\label{eq:relu}
G(\theta) = \sigma\circ(\mf W_n \sigma\circ(\mf W_{n-1}\cdots\sigma\circ(\mf W_1\theta))),
\end{equation}
where $\sigma(x) = \max(x,0)$, $\sigma\circ(\mf x)$ denotes the entry-wise application of $\sigma(\cdot)$, and 
$W_{i}\in\mathbb{R}^{d_{i}\times d_{i-1}}$ with $d_n = d$ and $d_i\leq d$.
It generates a high-dimensional vector $G( \theta ^*)\in\mathbb{R}^d$ from a low-dimensional signal $\theta^*\in\mathbb{R}^k$. 

For example, in neural nets based generative models such as generative adversarial nets (GANs) \cite{goodfellow2014generative} and variational auto encoders (VAEs) \cite{kingma2013auto}, the generator is responsible for generating high dimensional vectors in $\mathbb{R}^d$ that resemble the samples in the training image dataset from a low dimensional representation space via a deep neural network. Since the image samples are, more often than not, distributed close to a low-dimensional manifold of $\mathbb{R}^d$, a well-trained generative model is able to capture such a manifold structure, which can be difficult to represent in canonical basis otherwise.














==> xiaohan.tex <==
\newcommand{\rom}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\enas}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\ena}{\end{eqnarray}}
\newcommand{\bms}{\begin{multline*}}
\newcommand{\ems}{\end{multline*}}
\newcommand{\bels}{\begin{align*}}
\newcommand{\enls}{\end{align*}}
\newcommand{\bel}{\begin{align}}
\newcommand{\enl}{\end{align}}
\newcommand{\qmq}[1]{\quad \mbox{#1} \quad}
\newcommand{\qm}[1]{\quad \mbox{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\bbox}{\hfill $\Box$}
\newcommand{\ignore}[1]{}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\Bvert}{\left\vert\vphantom{\frac{1}{1}}\right.}
%perl texref.pl -unref cnm0616.tex > labelrefs
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{condition}{Condition}[section]
\newtheorem{assumption}{Assumption}[section]

\newcommand{\pf}{\noindent {\bf Proof:} }
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\newcommand{\lcolor}[1]{\textcolor{magenta}
	{#1}}  % Larry's colored text
\newcommand{\lcomm}[1]{\marginpar{\tiny\lcolor{#1}}}

\newcommand{\xcolor}[1]{\textcolor{blue}{#1}}
\newcommand{\xcomm}[1]{\marginpar{\tiny\xcolor{#1}}}

\newcommand{\expect}[1]{\mathbb{E}{\l[#1\r]}}





